Response-act Guided Reinforced Dialogue Generation for Mental Health Counseling

Virtual Mental Health Assistants (VMHAs) have become a prevalent method for receiving mental health counseling in the digital healthcare space. An assistive counseling conversation commences with natural open-ended topics to familiarize the client with the environment and later converges into more fine-grained domain-specific topics. Unlike other conversational systems, which are categorized as open-domain or task-oriented systems, VMHAs possess a hybrid conversational flow. These counseling bots need to comprehend various aspects of the conversation, such as dialogue-acts, intents, etc., to engage the client in an effective conversation. Although the surge in digital health research highlights applications of many general-purpose response generation systems, they are barely suitable in the mental health domain -- the prime reason is the lack of understanding in mental health counseling. Moreover, in general, dialogue-act guided response generators are either limited to a template-based paradigm or lack appropriate semantics. To this end, we propose READER -- a REsponse-Act guided reinforced Dialogue genERation model for the mental health counseling conversations. READER is built on transformer to jointly predict a potential dialogue-act d(t+1) for the next utterance (aka response-act) and to generate an appropriate response u(t+1). Through the transformer-reinforcement-learning (TRL) with Proximal Policy Optimization (PPO), we guide the response generator to abide by d(t+1) and ensure the semantic richness of the responses via BERTScore in our reward computation. We evaluate READER on HOPE, a benchmark counseling conversation dataset and observe that it outperforms several baselines across several evaluation metrics -- METEOR, ROUGE, and BERTScore. We also furnish extensive qualitative and quantitative analyses on results, including error analysis, human evaluation, etc.

==> Aseem_Ishan ReponseGen AAAI-_WWW/tables/data.tex <==

\begin{table}[!t]
\centering
\caption{Statistics of the HOPE dataset \cite{malhotra2021speaker}. The dyadic counseling conversational dataset contains a total of 12.8k utterances, each associated with one of the 12 dialogue-act labels.}
\label{tab:counts}
\scalebox{1.0}{
\begin{tabular}{l|cccc}
\toprule
HOPE & Train & Validation & Test & Total \\
\cmidrule{1-5}
Dialogue Sessions & 149 & 21 & 43 & 212\\
Client Utterances  & 4668 & 595 & 1119 & 6382\\
Therapist Utterances  & 4751 & 599 & 1122 & 6472\\
\cdashline{1-5}
\#Total Utterances & 9419 & 1194 & 2241 & 12854\\
\bottomrule
\end{tabular}
}
% \vspace{-7mm}
\end{table}

==> Aseem_Ishan ReponseGen AAAI-_WWW/tables/fullDialogExample.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/READER-complete.pdf}
    \label{tab:compdialogue}
    \caption{Generation of one complete counseling dialogue turn by turn by \model. We provide \model\ with initial sequence of utterances as an input context and model generates one turn at a time. We repeat this process with generated utterances as new inputs and shown below is a sample of dialogue generated by \model.}
\end{figure}


% --------



% \begin{table*}[h!]
% \label{tab:dialogueexample}
% \centering
% \label{tab:dialogueexample}
% \caption{Generation of one complete counseling dialogue turn by turn by \model. We provide \model\ with initial sequence of utterances as an input context and model generates one turn at a time. We repeat this process with generated utterances as new inputs and shown below is a sample of dialogue generated by \model.}
% % \vspace{-3mm}
% % \fontsize{6}{7}\selectfont
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c|p{58em}} \toprule
% \textbf{Conversation Type} & {\centering \textbf{Dialogue}} \\\cmidrule{1-2}
% Input Context & {\textbf{Therapist:} Hi George, how you doing today?}\\
%  & {\textbf{Client:} Okay.}\\
%  & {\textbf{Therapist:} I'd like to give you a test that measures your thinking and memory. Is that okay with you?}\\
%  & {\textbf{Client:} Yeah.}\\
%  & {\textbf{Therapist:} So ask if you have questions and if you could answer as best as you can that would appreciate.}\\
%  & {\textbf{Client:} Okay.}\\
%  & {\textbf{Therapist:} What's today's date?}\\
%  & {\textbf{Client:} 15th}\\
% & {\textbf{Therapist:}  That's good George thank you. I would like you to spell the word world backwards}\\ 
% \\
% \cdashline{1-2}
% \\
% \model\ Generated & \textbf{Client: } Yes i can.\\ 
% & \textbf{Therapist: } Thank you, George. This has been helpful. I appreciate you participating. I mean, I'm not great at this. But, I appreciate the effort you put into this. Can you explain your issues?\\
% & \textbf{Client: } I meant, of course, that at a certain point reaching for a drink becomes habit. You wake up every day and can't seem to get any work done without a drink. I feel so stressed after work.\\
% & \textbf{Therapist: } I suppose I just want to reassure you that it's absolutely normal to have feelings of depression and anxiety. It's really very common, and it certainly isn't auto strange at all. So I'm glad we were able to come to come here and talk about it, it's really important for us to have this talk.\\
% & \textbf{Client: } I see but this does not help me.\\
% & \textbf{Therapist: } So, did you tell me that you were indifferent to the drink? And why am I curious about that? Because usually, you’ve seemed to take issue with it. And now I’m curious as to whether that’s still the case.\\
% & \textbf{Client: } I guess I just don't know why I should keep living like this.\\
% & \textbf{Therapist: } You're fine. It is not quite as bad as its been before. You mentioned earlier that you've had ups and downs before\\

% \bottomrule
% \end{tabular}}
% \end{table*}

==> Aseem_Ishan ReponseGen AAAI-_WWW/tables/general.tex <==
\begin{table}[!t]\centering
% \vspace{-3mm}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|rrrrr}\toprule


Counselling Label &R-1 &R-2 &R-L &QAE &BS \\
\cmidrule{1-6}

\model\ $-$ SH $-$ PD & $20.92$ & $5.00$ & $7.44$ & $20.71$ & $0.0019$ \\

\model\ $-$ PD $-$ RT & $36.00$ & $9.00$ & $9.14$ & $20.47$ & $0.2032$ \\

\model\ $-$ RT $-$ SH & $28.63$ &$8.06$ & $9.55$ & $23.02$ & $-0.0209$ \\

\model\ $-$ SH & $39.77$ & $9.55$ & $8.98$ & $24.11$ & $0.1908$ \\

\model\ $-$ PD & $36.87$ & $10.02$ & $11.22$ & \bf 33.38 & $0.2420$ \\

\model\ $-$ RT & $42.01$ &$9.83$ & $16.50$ & $18.03$ & $0.2060$ \\

\model\ $-$ MH-Know $-$ CCC & $39.67$ &$9.95$ & $12.69$ & $21.19$ & $0.2003$ \\

\model\ $-$ MH-Know & $40.42$ &$10.09$ & $11.00$ & $23.97$ & $0.2429$ \\
\cdashline{1-6}
\model\ & \bf 45.36 & \bf 15.71 & \bf 24.75 & 25.42 & \bf 0.3407 \\

\bottomrule
\end{tabular}}
% \vspace{-7mm}
\caption{Ablation study on the effect of different modules of \model. SH, PD, DF and RT are psychotherapy elements. MH-Know and CCC are knowledge infused module and counseling component classifier module respectively. We present our analysis on five scores to understand all aspects of summary generation.}
\label{tab:ablation_result}

\end{table}

==> Aseem_Ishan ReponseGen AAAI-_WWW/tables/huma_eval.tex <==
\begin{table}[!t]
\centering
 % \vspace{-3mm}
\caption{Human evaluation on the responses generated from \model\  when compared to the top two best performing baselines. We observe that the performance of \model\ across all metrics is up to the mark and slightly better than the best-performing dialogue models. }
\label{tab:humaneval}
\scalebox{1.0}{
\begin{tabular}{l|cccc}
\toprule
Model & Relevance & Consistency & Fluency & Coherence \\
\cmidrule{1-5}
DialoGPT  & 2.11 & 2.42 & 2.90 & 2.30\\
GPT2  & 2.70 & 3.00 & 3.01 & 2.44\\
\cdashline{1-5}
\textbf{\model} & \bf 2.85 & \bf 3.05 & \bf 3.05 & \bf 2.95\\
\bottomrule
\end{tabular}
}

 \vspace{-5mm}
\end{table}

==> Aseem_Ishan ReponseGen AAAI-_WWW/tables/racHead.tex <==
\begin{table}[!t]
\centering
\caption{Performance of RAC-Head from \model.}

\scalebox{1.0}{
\begin{tabular}{l|cccc}
\toprule
Model & Precision & Recall & F1 & Accuracy\\
\cmidrule{1-5}
SOTA vs Gold Labels & 0.69 & 0.55 & 0.52 & 0.55\\
RAC-Head vs Gold Labels  & 0.49 & 0.49 & 0.42 & 0.49\\
RAC-Head vs SOTA  & 0.50 & 0.45 & 0.41 & 0.45\\
\bottomrule
\end{tabular}
}
% \vspace{-7mm}
\label{tab:rachead}
\end{table}


==> Aseem_Ishan ReponseGen AAAI-_WWW/tables/result.tex <==
\begin{table*}[t]\centering

\renewcommand*{\arraystretch}{1.0}
\caption{Results obtained on the HOPE dataset. We show ROUGE (1, 2, L), BERTScore (BS), and METEOR to assess the performance of the \model. $Rew(x)$ is the reward function, where $x$ is the parameter.}
\label{tab: results}
\resizebox{0.95\textwidth}{!}
{
\begin{tabular}{llcccccccccccc}


\toprule
& \multirow{2}{*}{} &\multicolumn{3}{c}{R1} &\multicolumn{3}{c}{R2} &\multicolumn{3}{c}{RL} &\multirow{2}{*}{BS} &\multirow{2}{*}{METEOR} \\\cmidrule{3-11}
& & P & R & F1 & P & R & F1 & P & R & F1 & & \\ \midrule
\multirow{7}{*}{\rotatebox{90}{Baselines}} & DialoGPT \cite{zhang-etal-2020-dialogpt} &12.34 &40.48 &15.72 &2.92 &11.83 &4.42 &12.23 &38.60 &15.76 &0.7603 &0.2021 \\
& GPT2 \cite{radford2019language} &12.70 & 32.63 & 14.98 & 3.08 & 7.92 & 3.51 & 13.74 & 32.05 & 15.87 & 0.7445 & 0.1754 \\
& DialogVED \cite{chen-etal-2022-dialogved} & 12.48 & 31.74 & 12.8 & 0.98 & 2.45 & 1.22 & 12.45 & 31.11 & 14.46 & 0.7189 & 0.2000 \\
& ProphetNet \cite{qi-etal-2021-prophetnet} &12.15 & 34.29 &14.48 & 3.30 &10.41 &4.17  & 12.24 & 33.12 & 15.18 & 0.6707 & 0.1901\\
& VHCR \cite{park-etal-2018-hierarchical} &11.29 & 21.33 &11.81 & 2.66 &3.49 &3.00  & 10.01 & 19.72 & 10.99 & 0.5953 & 0.1041\\
& HRED \cite{10.5555/3016387.3016435} & 11.52 & 21.51 & 10.72 & 1.89 & 6.42 & 2.92 & 12.12 & 24.36 & 13.56 & 0.6259 & 0.1425 \\
& HRED w/ Sp. Utt. Encoder \cite{https://doi.org/10.48550/arxiv.1907.05599} & 11.77 & 28.63 & 10.08 & 1.29 & 4.19 & 2.06 & 12.25 & 21.27 & 12.72 & 0.6171 & 0.1801\\

\midrule
\multirow{3}{*}{\rotatebox{90}{Ours}} & RagRes w/ DialoGPT &12.41  &43.91 &16.12 &3.70 &13.72 &4.98 &11.92 &41.02 &16.30 &0.7656 &0.2098 \\
& \model\ -- RAC-Head & 12.64 & 41.48 & 15.78 & 3.60 & 11.83 & 4.58 & 12.3 & 38.64 & 15.90 & 0.7628 & 0.2039 \\
% & \rowcolor{blue!20}
% \textbf{Ablations} & & & & & & & & & & & \\
&\bf \model &\textbf{12.82} &\textbf{43.93} &\textbf{16.15} &\textbf{3.77} &\textbf{13.67} &\textbf{4.93} &\textbf{12.51} &\textbf{40.82} &\textbf{16.32} &\textbf{0.7666} &\textbf{0.2103} \\
% \toprule
\midrule
% \textbf{Reward Ablation} & & & & & & & & & & & \\
\multirow{5}{*}{\rotatebox{90}{Ablations}} & $\qquad$ -- $Rew($R$)$ & $11.73$ & $38.82$ & $14.65$& 2.28 &$8.45$&$2.96$& 11.21 &35.76&14.53&0.7561&0.1840 \\
& $\qquad$ -- $Rew($RAC$)$ &12.36 &40.71 &15.43 &3.13 &11.12 &4.06 &11.91 &37.63 &15.40 &0.7609 &0.2000 \\
& $\qquad$ -- $Rew($RAC + R$)$ &11.92 &38.06 &14.70 &2.43 &8.26 &3.11 &11.40 & 34.98 &14.58 &0.7530 &0.1874 \\
& $\qquad$ -- $Rew($R + BS$)$ &12.48 &41.13&15.57 &3.52 &11.85 &4.47&12.22 &38.29 &15.77 &0.7527 &0.2092 \\
& $\qquad$ -- $Rew($RAC + BS$)$ & 12.01 & 40.45 & 15.18 & 2.72 & 9.93 & 3.52 & 11.46 & 37.05 & 14.97 & 0.7577 & 0.1908 \\
% \model\ w/ Rew(R+DAC +BS only) & & & & & & & & & & & \\
\midrule
& $\Delta_{\model-BEST}(\%)$ & \textcolor{blue}{$\uparrow 0.94$} & \textcolor{blue}{$\uparrow 8.5$} & \textcolor{blue}{$\uparrow 2.73$} & \textcolor{blue}{$\uparrow 14.24$} & \textcolor{blue}{$\uparrow 15.50$} & \textcolor{blue}{$\uparrow 11.53$} & \textcolor{red}{$\downarrow 8.90$}& \textcolor{blue}{$\uparrow 5.69$} & \textcolor{blue}{$\uparrow 2.83$} & \textcolor{blue}{$\uparrow 0.82$} & \textcolor{blue}{$\uparrow 4.05$} \\ 

\bottomrule

\end{tabular}}

\end{table*}

==> Aseem_Ishan ReponseGen AAAI-_WWW/tables/swda.tex <==
\begin{table*}[!t]\centering
\footnotesize
% \scriptsize
% \renewcommand*{\arraystretch}{1.0}
\caption{Results obtained on the Switchboard Dialogue-act dataset. We show Rouge (1, 2, L), BERTScore (BS), and Meteor to assess the generalizability of the \model\ on datasets similar to HOPE.}
\label{tab: swda}
\resizebox{\textwidth}{!}
{
\begin{tabular}{lcccccccccccc}\toprule
\multirow{2}{*}{} &\multicolumn{3}{c}{R1} &\multicolumn{3}{c}{R2} &\multicolumn{3}{c}{RL} &\multirow{2}{*}{BertScore} &\multirow{2}{*}{Meteor} \\\cmidrule{2-10}
& P & R & F1 & P & R & F1 & P & R & F1 & & \\\midrule
DialoGPT &21.64 &27.16 &23.87 &11.41 &14.43 &12.47 &19.53 &23.78 &21.46 &0.6615 &0.1836 \\
GPT2 & 22.25 &27.95 &24.14 &11.89 &14.49 &12.75 &20.12 &24.76 &21.80 &0.6608 &0.1822 \\
\midrule
\rowcolor{blue!20}
\bf \model & 22.32 &27.92 &24.18 &11.97 &14.49 &12.79 &20.20 &24.76 &21.84 & 0.7295 & 0.1850\\

\midrule
$\Delta_{\model-BEST}(\%)$ & \textcolor{blue}{$\uparrow 0.3$} & \textcolor{red}{$\downarrow 0.1$} & \textcolor{blue}{$\uparrow 0.1$} & \textcolor{blue}{$\uparrow 0.6$} & \textcolor{blue}{$\uparrow 0.0$} & \textcolor{blue}{$\uparrow 0.3$} & \textcolor{blue}{$\uparrow 0.3$}& \textcolor{blue}{$\uparrow 0.0$} & \textcolor{blue}{$\uparrow 0.1$} & \textcolor{blue}{$\uparrow 9.4$} & \textcolor{blue}{$\uparrow 1.5$}  \\

\bottomrule
\end{tabular}}

\end{table*}

==> Aseem_Ishan ReponseGen AAAI-_WWW/tables/therapistGen.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/READER-therapist.pdf}
    \label{tab:dialoguecomplete}
    \caption{A complete dialogue conversation generated by the model, \model. The dialogue shows part of utterances from actual conversation and then shows the responses generated considering the previous few utterances as context.}
\end{figure}


% \begin{table*}[h!]
% \label{tab:dialogueexample}
% \centering
% \label{tab:dialogueexample}
% \caption{In this table, we present a complete dialogue conversation generated by the model, \model. The dialogue shows part of utterances from actual conversation and then shows the responses generated considering the previous few utterances as context.}
% % \vspace{-3mm}
% % \fontsize{6}{7}\selectfont
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|p{58em}|l} \toprule
% \textbf{Conversation Type} & {\centering \textbf{Dialogue}} \\\midrule
% Therapist & & Client \\
% \multicolumn{2}{l}{\multirow{1}{60em}{Robert Smith, thank you for coming to see me say,I,m Dr. Stanley. I'm one of the doctors that works here. Obviously anything that we say is confidential between us and the team that I work with a new GP who's asked me to see you. I hear there have been some problems with your housing. Do you want to tell me a little bit about it?}} & \\ \\ \\
%  & \multicolumn{2}{l}{\multirow{1}{60em}{Yeah, I've had all sorts of problems. I mean,where do you want me to start? neighbors police. People spying on me in my street. You know, none of them admit to it. But I that you know, my neighbors they, but it's my it's mainly them at number nine. But I've seen them talking to the ones that number six and across the road as well.}}\\ \\ \\
% \multicolumn{2}{l}{\multirow{1}{60em}{You know, so what, when did things start to go wrong?}} & \\ 
% \cdashline{1-2}
% \model\ Generated & \textbf{Client: } Well, it's it's the harassment. It's the spying on me in my street. You know that\\ 
% % \hline
% \cdashline{1-2}
% Actual Conversation &\textbf{Therapist: } What makes you think they want you out the street? \\
% \cdashline{1-2}
% \model\ Generated & \textbf{Client: } I thought maybe someone else had a big problem with my attention. And I guess found the time where my attention was coming from.\\ 
% \cdashline{1-2}

% Actual Conversation & \textbf{Therapist: } Why do you think they're doing that? \\
% \cdashline{1-2}

% \model\ Generated & \textbf{Client: } Well, nobody told me.\\
% & \textbf{Therapist: } You said your phone was clicking What was that about?\\
% & \textbf{Client: } Well, I can hear him next door. Always on the phone again, always\\
% \cdashline{1-2}

% Actual Conversation & \textbf{Therapist: } Any other explanation for that? \\
% \cdashline{1-2}

% \model\ Generated & \textbf{Client: } I'm definitely confused. And I think they're getting on me. But you know, I've been very difficult to do it. I'm just\\

% \cdashline{1-2}
% Actual Conversation & \textbf{Therapist: } 
% Okay, so just to summarize at this point, your your phones Something's happening to telephone, you can hear your neighbors talking about what you're doing, making a commentary on your actions every day, every day. And you feel that there's some sort of reason for their actions doing this. Any other things that you've got problems with?\\
% \hline{1-2}

% \model\ Generated & \textbf{Client: } So they started properly, like deciding that they wanted, they wanted me out of the street. And when I was there in the street people came by.  Well, yeah, I mean, I've been thinking about killing myself seriously wrong. And I'm scared. \\

% \bottomrule
% \end{tabular}}

% \end{table*}




% \begin{table*}[h!]
% \label{tab:dialogueexample}
% \centering
% \label{tab:dialogueexample}
% \caption{In this table, we present a complete dialogue conversation generated by the model, \model. The dialogue shows part of utterances from actual conversation and then shows the responses generated considering the previous few utterances as context.}
% % \vspace{-3mm}
% % \fontsize{6}{7}\selectfont
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c|p{58em}} \toprule
% \textbf{Conversation Type} & {\centering \textbf{Dialogue}} \\\cmidrule{1-2}
% Actual Conversation & {\textbf{Therapist:} Robert Smith, thank you for coming to see me say,I,m Dr. Stanley. I'm one of the doctors that works here. Obviously anything that we say is confidential between us and the team that I work with a new GP who's asked me to see you. I hear there have been some problems with your housing. Do you want to tell me a little bit about it?}\\
%  & {\textbf{Client:} Yeah, I've had all sorts of problems. I mean,where do you want me to start? neighbors police. People spying on me in my street. You know, none of them admit to it. But I that you know, my neighbors they, but it's my it's mainly them at number nine. But I've seen them talking to the ones that number six and across the road as well.}\\ 
%  & \textbf{Therapist: }  You know, so what, when did things start to go wrong? \\ 
% \cdashline{1-2}
% \model\ Generated & \textbf{Client: } Well, it's it's the harassment. It's the spying on me in my street. You know that\\ 
% % \hline
% \cdashline{1-2}
% Actual Conversation &\textbf{Therapist: } What makes you think they want you out the street? \\
% \cdashline{1-2}
% \model\ Generated & \textbf{Client: } I thought maybe someone else had a big problem with my attention. And I guess found the time where my attention was coming from.\\ 
% \cdashline{1-2}

% Actual Conversation & \textbf{Therapist: } Why do you think they're doing that? \\
% \cdashline{1-2}

% \model\ Generated & \textbf{Client: } Well, nobody told me.\\
% & \textbf{Therapist: } You said your phone was clicking What was that about?\\
% & \textbf{Client: } Well, I can hear him next door. Always on the phone again, always\\
% \cdashline{1-2}

% Actual Conversation & \textbf{Therapist: } Any other explanation for that? \\
% \cdashline{1-2}

% \model\ Generated & \textbf{Client: } I'm definitely confused. And I think they're getting on me. But you know, I've been very difficult to do it. I'm just\\

% \cdashline{1-2}
% Actual Conversation & \textbf{Therapist: } 
% Okay, so just to summarize at this point, your your phones Something's happening to telephone, you can hear your neighbors talking about what you're doing, making a commentary on your actions every day, every day. And you feel that there's some sort of reason for their actions doing this. Any other things that you've got problems with?\\
% \hline{1-2}

% \model\ Generated & \textbf{Client: } So they started properly, like deciding that they wanted, they wanted me out of the street. And when I was there in the street people came by.  Well, yeah, I mean, I've been thinking about killing myself seriously wrong. And I'm scared. \\

% \bottomrule
% \end{tabular}}

% \end{table*}


==> tables/fullDialogExample.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/READER-complete.pdf}
    \label{tab:compdialogue}
    \caption{Generation of one complete counseling dialogue turn by turn by \model. We provide \model\ with initial sequence of utterances as an input context and model generates one turn at a time. We repeat this process with generated utterances as new inputs and shown below is a sample of dialogue generated by \model.}
\end{figure}


% --------



% \begin{table*}[h!]
% \label{tab:dialogueexample}
% \centering
% \label{tab:dialogueexample}
% \caption{Generation of one complete counseling dialogue turn by turn by \model. We provide \model\ with initial sequence of utterances as an input context and model generates one turn at a time. We repeat this process with generated utterances as new inputs and shown below is a sample of dialogue generated by \model.}
% % \vspace{-3mm}
% % \fontsize{6}{7}\selectfont
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c|p{58em}} \toprule
% \textbf{Conversation Type} & {\centering \textbf{Dialogue}} \\\cmidrule{1-2}
% Input Context & {\textbf{Therapist:} Hi George, how you doing today?}\\
%  & {\textbf{Client:} Okay.}\\
%  & {\textbf{Therapist:} I'd like to give you a test that measures your thinking and memory. Is that okay with you?}\\
%  & {\textbf{Client:} Yeah.}\\
%  & {\textbf{Therapist:} So ask if you have questions and if you could answer as best as you can that would appreciate.}\\
%  & {\textbf{Client:} Okay.}\\
%  & {\textbf{Therapist:} What's today's date?}\\
%  & {\textbf{Client:} 15th}\\
% & {\textbf{Therapist:}  That's good George thank you. I would like you to spell the word world backwards}\\ 
% \\
% \cdashline{1-2}
% \\
% \model\ Generated & \textbf{Client: } Yes i can.\\ 
% & \textbf{Therapist: } Thank you, George. This has been helpful. I appreciate you participating. I mean, I'm not great at this. But, I appreciate the effort you put into this. Can you explain your issues?\\
% & \textbf{Client: } I meant, of course, that at a certain point reaching for a drink becomes habit. You wake up every day and can't seem to get any work done without a drink. I feel so stressed after work.\\
% & \textbf{Therapist: } I suppose I just want to reassure you that it's absolutely normal to have feelings of depression and anxiety. It's really very common, and it certainly isn't auto strange at all. So I'm glad we were able to come to come here and talk about it, it's really important for us to have this talk.\\
% & \textbf{Client: } I see but this does not help me.\\
% & \textbf{Therapist: } So, did you tell me that you were indifferent to the drink? And why am I curious about that? Because usually, you’ve seemed to take issue with it. And now I’m curious as to whether that’s still the case.\\
% & \textbf{Client: } I guess I just don't know why I should keep living like this.\\
% & \textbf{Therapist: } You're fine. It is not quite as bad as its been before. You mentioned earlier that you've had ups and downs before\\

% \bottomrule
% \end{tabular}}
% \end{table*}

==> tables/general.tex <==
\begin{table}[!t]\centering
% \vspace{-3mm}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|rrrrr}\toprule


Counselling Label &R-1 &R-2 &R-L &QAE &BS \\
\cmidrule{1-6}

\model\ $-$ SH $-$ PD & $20.92$ & $5.00$ & $7.44$ & $20.71$ & $0.0019$ \\

\model\ $-$ PD $-$ RT & $36.00$ & $9.00$ & $9.14$ & $20.47$ & $0.2032$ \\

\model\ $-$ RT $-$ SH & $28.63$ &$8.06$ & $9.55$ & $23.02$ & $-0.0209$ \\

\model\ $-$ SH & $39.77$ & $9.55$ & $8.98$ & $24.11$ & $0.1908$ \\

\model\ $-$ PD & $36.87$ & $10.02$ & $11.22$ & \bf 33.38 & $0.2420$ \\

\model\ $-$ RT & $42.01$ &$9.83$ & $16.50$ & $18.03$ & $0.2060$ \\

\model\ $-$ MH-Know $-$ CCC & $39.67$ &$9.95$ & $12.69$ & $21.19$ & $0.2003$ \\

\model\ $-$ MH-Know & $40.42$ &$10.09$ & $11.00$ & $23.97$ & $0.2429$ \\
\cdashline{1-6}
\model\ & \bf 45.36 & \bf 15.71 & \bf 24.75 & 25.42 & \bf 0.3407 \\

\bottomrule
\end{tabular}}
% \vspace{-7mm}
\caption{Ablation study on the effect of different modules of \model. SH, PD, DF and RT are psychotherapy elements. MH-Know and CCC are knowledge infused module and counseling component classifier module respectively. We present our analysis on five scores to understand all aspects of summary generation.}
\label{tab:ablation_result}

\end{table}

==> tables/racHead.tex <==
\begin{table}[!t]
\centering
\caption{Performance of RAC-Head from \model.}

\scalebox{1.0}{
\begin{tabular}{l|cccc}
\toprule
Model & Precision & Recall & F1 & Accuracy\\
\cmidrule{1-5}
SOTA vs Gold Labels & 0.69 & 0.55 & 0.52 & 0.55\\
RAC-Head vs Gold Labels  & 0.49 & 0.49 & 0.42 & 0.49\\
RAC-Head vs SOTA  & 0.50 & 0.45 & 0.41 & 0.45\\
\bottomrule
\end{tabular}
}
% \vspace{-7mm}
\label{tab:rachead}
\end{table}


==> tables/therapistGen.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/READER-therapist.pdf}
    \label{tab:dialoguecomplete}
    \caption{A complete dialogue conversation generated by the model, \model. The dialogue shows part of utterances from actual conversation and then shows the responses generated considering the previous few utterances as context.}
\end{figure}


% \begin{table*}[h!]
% \label{tab:dialogueexample}
% \centering
% \label{tab:dialogueexample}
% \caption{In this table, we present a complete dialogue conversation generated by the model, \model. The dialogue shows part of utterances from actual conversation and then shows the responses generated considering the previous few utterances as context.}
% % \vspace{-3mm}
% % \fontsize{6}{7}\selectfont
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|p{58em}|l} \toprule
% \textbf{Conversation Type} & {\centering \textbf{Dialogue}} \\\midrule
% Therapist & & Client \\
% \multicolumn{2}{l}{\multirow{1}{60em}{Robert Smith, thank you for coming to see me say,I,m Dr. Stanley. I'm one of the doctors that works here. Obviously anything that we say is confidential between us and the team that I work with a new GP who's asked me to see you. I hear there have been some problems with your housing. Do you want to tell me a little bit about it?}} & \\ \\ \\
%  & \multicolumn{2}{l}{\multirow{1}{60em}{Yeah, I've had all sorts of problems. I mean,where do you want me to start? neighbors police. People spying on me in my street. You know, none of them admit to it. But I that you know, my neighbors they, but it's my it's mainly them at number nine. But I've seen them talking to the ones that number six and across the road as well.}}\\ \\ \\
% \multicolumn{2}{l}{\multirow{1}{60em}{You know, so what, when did things start to go wrong?}} & \\ 
% \cdashline{1-2}
% \model\ Generated & \textbf{Client: } Well, it's it's the harassment. It's the spying on me in my street. You know that\\ 
% % \hline
% \cdashline{1-2}
% Actual Conversation &\textbf{Therapist: } What makes you think they want you out the street? \\
% \cdashline{1-2}
% \model\ Generated & \textbf{Client: } I thought maybe someone else had a big problem with my attention. And I guess found the time where my attention was coming from.\\ 
% \cdashline{1-2}

% Actual Conversation & \textbf{Therapist: } Why do you think they're doing that? \\
% \cdashline{1-2}

% \model\ Generated & \textbf{Client: } Well, nobody told me.\\
% & \textbf{Therapist: } You said your phone was clicking What was that about?\\
% & \textbf{Client: } Well, I can hear him next door. Always on the phone again, always\\
% \cdashline{1-2}

% Actual Conversation & \textbf{Therapist: } Any other explanation for that? \\
% \cdashline{1-2}

% \model\ Generated & \textbf{Client: } I'm definitely confused. And I think they're getting on me. But you know, I've been very difficult to do it. I'm just\\

% \cdashline{1-2}
% Actual Conversation & \textbf{Therapist: } 
% Okay, so just to summarize at this point, your your phones Something's happening to telephone, you can hear your neighbors talking about what you're doing, making a commentary on your actions every day, every day. And you feel that there's some sort of reason for their actions doing this. Any other things that you've got problems with?\\
% \hline{1-2}

% \model\ Generated & \textbf{Client: } So they started properly, like deciding that they wanted, they wanted me out of the street. And when I was there in the street people came by.  Well, yeah, I mean, I've been thinking about killing myself seriously wrong. And I'm scared. \\

% \bottomrule
% \end{tabular}}

% \end{table*}




% \begin{table*}[h!]
% \label{tab:dialogueexample}
% \centering
% \label{tab:dialogueexample}
% \caption{In this table, we present a complete dialogue conversation generated by the model, \model. The dialogue shows part of utterances from actual conversation and then shows the responses generated considering the previous few utterances as context.}
% % \vspace{-3mm}
% % \fontsize{6}{7}\selectfont
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c|p{58em}} \toprule
% \textbf{Conversation Type} & {\centering \textbf{Dialogue}} \\\cmidrule{1-2}
% Actual Conversation & {\textbf{Therapist:} Robert Smith, thank you for coming to see me say,I,m Dr. Stanley. I'm one of the doctors that works here. Obviously anything that we say is confidential between us and the team that I work with a new GP who's asked me to see you. I hear there have been some problems with your housing. Do you want to tell me a little bit about it?}\\
%  & {\textbf{Client:} Yeah, I've had all sorts of problems. I mean,where do you want me to start? neighbors police. People spying on me in my street. You know, none of them admit to it. But I that you know, my neighbors they, but it's my it's mainly them at number nine. But I've seen them talking to the ones that number six and across the road as well.}\\ 
%  & \textbf{Therapist: }  You know, so what, when did things start to go wrong? \\ 
% \cdashline{1-2}
% \model\ Generated & \textbf{Client: } Well, it's it's the harassment. It's the spying on me in my street. You know that\\ 
% % \hline
% \cdashline{1-2}
% Actual Conversation &\textbf{Therapist: } What makes you think they want you out the street? \\
% \cdashline{1-2}
% \model\ Generated & \textbf{Client: } I thought maybe someone else had a big problem with my attention. And I guess found the time where my attention was coming from.\\ 
% \cdashline{1-2}

% Actual Conversation & \textbf{Therapist: } Why do you think they're doing that? \\
% \cdashline{1-2}

% \model\ Generated & \textbf{Client: } Well, nobody told me.\\
% & \textbf{Therapist: } You said your phone was clicking What was that about?\\
% & \textbf{Client: } Well, I can hear him next door. Always on the phone again, always\\
% \cdashline{1-2}

% Actual Conversation & \textbf{Therapist: } Any other explanation for that? \\
% \cdashline{1-2}

% \model\ Generated & \textbf{Client: } I'm definitely confused. And I think they're getting on me. But you know, I've been very difficult to do it. I'm just\\

% \cdashline{1-2}
% Actual Conversation & \textbf{Therapist: } 
% Okay, so just to summarize at this point, your your phones Something's happening to telephone, you can hear your neighbors talking about what you're doing, making a commentary on your actions every day, every day. And you feel that there's some sort of reason for their actions doing this. Any other things that you've got problems with?\\
% \hline{1-2}

% \model\ Generated & \textbf{Client: } So they started properly, like deciding that they wanted, they wanted me out of the street. And when I was there in the street people came by.  Well, yeah, I mean, I've been thinking about killing myself seriously wrong. And I'm scared. \\

% \bottomrule
% \end{tabular}}

% \end{table*}

